Counting Signed Vexillary Permutations

We show that the number of signed permutations avoiding 1234 equals the number of signed permutations avoiding 2143 (also called vexillary signed permutations), resolving a conjecture by Anderson and Fulton. The main tool that we use is the generating tree developed by West. Many further directions are mentioned in the end.

==> Sections-Vexillary/Section-Tree.tex <==
\section{Generating trees for 1234 and 2143 avoiding permutations}\label{sec:suc}

We will start working towards an explicit generating tree for $B^j_n(1234)$ and $B^j_n(2143)$ by first proving a lemma about the structure of a permutation that avoids either pattern. Throughout the discussion, the reader is invited to keep the following visualization of signed permutations in mind. A signed permutation $w$ can be represented by a point graph, where the $x$ axis corresponds to the indices $(-n, \ldots, -1, 1, \ldots n)$, and the $y$ axis corresponds to the images $(-n, \ldots, -1, 1, \ldots, n)$. A point appears at $(x,y)$ if the index $x$ is sent to the image $y$ by the signed permutation $w$. An example is shown in Figure \ref{fig:pointgraph}.

\begin{figure}[h!]
\centering
\begin{tikzpicture}[scale=0.6]
\draw[very thick](0,-5)--(0,5);
\draw[very thick](-5,0)--(5,0);
\node at (-4,-3) {$\bullet$};
\node at (-3,4) {$\bullet$};
\node at (-2,2) {$\bullet$};
\node at (-1,1) {$\bullet$};
\node at (1,-1) {$\bullet$};
\node at (2,-2) {$\bullet$};
\node at (3,-4) {$\bullet$};
\node at (4,3) {$\bullet$};
\end{tikzpicture}
\caption{The point graph of $\begin{matrix} -4 & -3 & -2 & -1 & 1 & 2 & 3 & 4 \\ -3 & 4 & 2 & 1 & -1 & -2 & -4 & 3 \end{matrix} $}
\label{fig:pointgraph}
\end{figure}

We will consider the cases of $2143$ and $1234$ in parallel.
\begin{lemma}\label{lem:struc}\leavevmode
\begin{enumerate}
    \item Suppose $w\in B_n^j(2143)$, where the $j$ positive indices with positive images are $1\leq i_1<i_2<\ldots<i_j\leq n$. Then $w(i_1)<w(i_2)<\ldots <w(i_j)$. 

    \item Suppose $w\in B_n^j(1234)$, where the $j$ positive indices with positive images are $1\leq i_1<i_2<\ldots<i_j\leq n$. Then $w(i_1)>w(i_2)>\ldots>w(i_j)$.
\end{enumerate}
\end{lemma}

In terms of the point graph of $w$, this lemma is saying that the $j$ points in the top right quadrant form an increasing sequence for $2143$, and a decreasing sequence for $1234$. And therefore, this is also true in the bottom left quadrant. This can be seen in Figure \ref{fig:struc}.

\begin{figure}[h!]
\centering
\begin{minipage}[b]{.45\textwidth}
\begin{tikzpicture}[scale=0.5]
\draw[very thick](0,-6)--(0,6);
\draw[very thick](-6,0)--(6,0);
\node at (-5,-5) {$\bullet$};
\node at (-4,-4) {$\bullet$};
\node at (-3,-3) {$\bullet$};
\node at (-2,-2) {$\bullet$};
\node at (-1,-1) {$\bullet$};
\node at (1,1) {$\bullet$};
\node at (2,2) {$\bullet$};
\node at (3,3) {$\bullet$};
\node at (4,4) {$\bullet$};
\node at (5,5) {$\bullet$};
\node at (5.5,2.5) {$j=5$};
\node at (0, -7) {$2143$};
\end{tikzpicture}



\end{minipage}\hfill
\begin{minipage}[b]{.45\textwidth}
\begin{tikzpicture}[scale=0.5]
\draw[very thick](0,-6)--(0,6);
\draw[very thick](-6,0)--(6,0);
\node at (-5,-1) {$\bullet$};
\node at (-4,-2) {$\bullet$};
\node at (-3,-3) {$\bullet$};
\node at (-2,-4) {$\bullet$};
\node at (-1,-5) {$\bullet$};
\node at (1,5) {$\bullet$};
\node at (2,4) {$\bullet$};
\node at (3,3) {$\bullet$};
\node at (4,2) {$\bullet$};
\node at (5,1) {$\bullet$};
\node at (5.5,4) {$j=5$};
\node at (0, -7) {$1234$};
\end{tikzpicture}

\end{minipage}
     
    \caption{Two quadrants of $2143$ and $1234$ avoiding permutations}
    \label{fig:struc}
\end{figure}

\begin{proof}\leavevmode
\begin{enumerate}
    \item Suppose not. Then there exists a pair of positive indices $i<j$ with $1\leq w(j)<w(i)\leq n$. Consider the pattern forming at the indices $-j, -i, i, j$. We have $w(-i)<w(-j)<0<w(j)<w(i)$, or in other words, the pattern is $2143$. This is a contradiction with $w\in B_n^j(2143)$.
    \item Analogous.
\end{enumerate}

\end{proof}



To motivate our method of generating signed permutations, let us first informally discuss how one can take an ordinary permutation and generate new permutations from it by simple operations. This discussion builds on \cite{west1995generating}. We will consider inserting one element to the previous permutation. For a permutation on $n$ indices, we will call the $n+1$ positions between indices \emph{sites}. One can consider inserting a new element to any site. In general, this new element can also get any image between $1$ and $n+1$. If we choose the image of the new element to be $i$, then all other images greater or equal to $i$ will get increased by one -- we think of this as making the image of the new element lie in the \emph{gap} between the previous $i-1$ and $i$. In terms of the point graph, we are inserting a point with an $x$ coordinate between the $x$ coordinates of two previously consecutive points (this is the site) and with a $y$ coordinate between two previously consecutive $y$ coordinates (this is the gap). In a specific scenario, one might want this generating procedure to be more constrained than just inserting any image to any site, in order to satisfy some additional properties.

With these preliminary considerations in mind, let us discuss what the generating procedure might be for our particular case. As we are dealing with signed permutations, our steps are not going to be adding just one new index and image, as this would violate the condition that the images of $i$ and $-i$ are negatives of each other, so we would not end up with signed permutations. Instead, we will simultaneously be inserting to the site $i$ and to the site $-i$, with images that are also negatives of each other. As we want to keep $j$, the number of positive indices with positive images, fixed, the only insertions we will perform are insertions of positive images to negative indices. Given these informal considerations, we will now finally formally define what we mean by insertions from now on. Nevertheless, the reader is invited to just think of insertions in terms of inserting points in the dot graph, as this definition is equivalent.

\begin{definition}
We define the following auxiliary function (one should think of this as the function pushing images to their new locations when the gap between $\ell-1$ and $\ell$ gets a new image):
\[\beta_\ell(x)= 
  \begin{cases} 
   x & \text{if } |x|<\ell \\
   x-1 & \text{if } x<-\ell\\
   x+1 & \text{if } x>\ell\\
  \end{cases}.\]
  
For a signed permutation $w$ on the indices $-n, \ldots, -1, 1, n$, let $w^{-i}_\ell$ be the signed permutation with the following first half (which uniquely determines the second half): \[\begin{matrix}   -(n{+}1) & -n &\ldots & -(i{+}1)& -i & -(i{-}1)&\ldots & -1\\
 \beta_\ell(w({-}n)) & \beta_\ell(w({-}(n{-}1)) &\ldots & \beta_\ell(w({-}i))& \ell & \beta_\ell(w({-}(i{-}1)))&\ldots & \beta_\ell(w({-}1)).\\ \end{matrix}\]
 
We call this inserting a new element to the site $-i$ and gap $\ell$. 
\end{definition}

On any step, we will be allowed to insert a new element to any negative index site. Furthermore, we want there to be at most one way to generate each permutation. For this reason, we will only ever add images that are larger than the current largest image among negative indices. Finally, we would like all the generated permutations to avoid $2143$ (or $1234$), and to generate all permutations avoiding $2143$ (or $1234$) To this end, we will only be performing an operation if the resulting permutation avoids $2143$ (or $1234$). Our start point will be a permutation with exactly $j$ positive indices with positive images, and no other positive indices. Such a permutation is unique by Lemma \ref{lem:struc}. In terms of our point graph representation, the points in the top right and bottom left quadrant are fixed, and all the action happens in the other two quadrants. The element we will be adding will always be the largest in the top left quadrant, and we will allow insertions to any site on the left. As for which gap the image of the new index falls in, we can think of the $j$ initial points as cutting the top left quadrant into $j+1$ layers. When we inserted the previous point to some layer, we can attach the next one to the same layer or any layer above it. Initially, we can insert a point to any layer.

To summarize what we have arrived at, let us finally explicitly define our pattern avoidance tree.

\begin{definition}\label{def:tree} 
For $\pi=1234$ or $\pi=2143$, define $BT^j(\pi)$, the signed permutation pattern avoidance tree for fixed number of positive indices with positive images $j$ to be the following generating tree:
\begin{itemize}
    \item The label of the root is the unique signed permutation on the indices $-j, \ldots, -1, 1, \ldots, j$ with  all positive indices sent to positive images. For $\pi=2143$, the root is \[\begin{matrix}   -j & \ldots & -1 & 1 & \ldots & j\\
    -j & \ldots & -1 & 1 & \ldots & j\\\end{matrix}\]
    For $\pi=1234$, the root is 
    \[\begin{matrix}  -j & \ldots & -1 & 1 & \ldots & j\\ -1 & \ldots & -j & j & \ldots & 1\\
    \end{matrix}\]
    \item The succession rule is the following. Our label is the permutation $w\in B_n$. Let $m$ be the maximal image of a negative index in $w$ ($m=0$ if there are no images). Let $X(w)$ be the set of $w^{-i}_\ell$ for all pairs $i,\ell$ with $1\leq n+1$ and $m<\ell\leq n+1$. The successor set of $w$ is the subset of $X(w)$ consisting of those permutations that avoid $\pi$.
\end{itemize}
\end{definition}



Let us confirm that this tree has the desired properties. Well, given a permutation avoiding $\pi=1234$ with $j$ positive indices with positive images, there is a way to reconstruct it by a sequence of such insertions. Any subpermutation of a permutation avoiding $1234$ also avoids $1234$. We start at the root of our tree, and then on each step we take the smallest image from our permutation that has not been inserted yet, and insert it in the tree. Each step can be made, as we are always inserting the new largest image to a negative index, and with the prescribed insertion we always end up with a signed permutation avoiding $1234$. For each permutation avoiding $1234$ and with $j$ positive indices with positive images, the way it can be constructed with our procedure is unique, as the only way is to start with the permutation containing only the positive images of positive indices, and to fill everything else in in increasing order. Additionally, as we add one index on each step, $B_n^j(\pi)$ as defined before is precisely the set of labels appearing on the $n-j$'th layer of the tree, where counting starts at $0$ from the layer of the root.

Our next goal is to give an alternative description of this tree that is easier to analyze. As the first step towards this goal, we have the following lemma that lets us ignore the bottom right quadrant.

\begin{lemma}\label{lem:ignore}
The following holds for $\pi\in \{2143, 1234\}$. For a vertex labelled $w$ in $BT^j(\pi)$, if a signed permutation $x$ in $X(w)$ contains $\pi$, then it contains some $\pi$ at indices $i_1, i_2, i_3, i_4$, such that there is no $i_k$ for which $i_k>0$, $x(i_k)<0$.
\end{lemma}

\begin{proof}

Say for a contradiction that $x$ contains $\pi$ but only so that it involves a positive index with a negative image. Let the indices at which one such $\pi$ appears be $a_1, a_2, a_3, a_4$. Consider the pattern appearing at the reflection of those images, that is, at $-a_4, -a_3, -a_2, -a_1$. It is easy to check explicitly that the pattern appearing at these indices is also $\pi$ (this is not true in general, but it is true for $\pi\in\{2143, 1234\}$). For these indices, we know that one of them is the reflection of a positive index with a negative image, so that one is a negative index with a positive image. By our assumption, we also know that this pattern contains a positive index with a negative image. As the negative index must come before the positive one in the pattern and this pair forms a decreasing sequence, the pair must correspond to a decreasing pair in $\pi$. We will now consider the two cases.
\begin{itemize}
    \item[$\pi=2143$:] This pair can either be $21$ or $43$. If this pair is $21$, then we would need to have a $43$ after the positive index with a negative image. Hence, this $43$ would come at positive indices. As our $2$ is a positive image, the $43$ also needs to come at positive images. But this is already a contradiction, as there is no pair of positive indices with decreasing positive images, as $w$ avoids $2143$, and the positive indices with positive images are not changed by the insertion, so Lemma \ref{lem:struc} applies. If this pair is $43$, we would similarly have to have a $21$ in the bottom left quadrant, which is impossible.
    \item[$\pi=1234$:] There is no decreasing pair in $1234$, so this is impossible.
\end{itemize}

\end{proof}


We still need some more terminology before getting to presenting the generating tree. The following three permutation statistics will be important.
\begin{itemize}
    \item {\bf The number of sites before the first ascent (or descent).} For a signed permutation $w$, by a site before the first ascent (descent) we mean a site such that there is no increasing (decreasing) pair of images among the indices before this site. When $w$ is clear from the context, we write $x$ for the number of sites before the first ascent (descent). We say a site is after the first ascent (descent) if it is not before the first ascent (descent).
    \item {\bf The number of active sites.} For a signed permutation $w$, we say a site with a negative index is \emph{active} with respect to a fixed pattern $\pi$ and some fixed gap $\ell$ if inserting an element to the gap $\ell$ in that site in $w$ results in a permutation that avoids $\pi$. When $\pi$, $w$, and $\ell$ are clear from the context, we will write $y$ for the number of active sites.
    \item {\bf The layer number.} As discussed before, the $j$ positive indices with positive images partition the gaps between images to $j+1$ sections or layers. Visually, this corresponds to the top left quadrant being partitioned into $j+1$ horizontal strips by horizontal lines passing through the points corresponding to positive indices with positive images. For a permutation $w$, the layer number is the number of layers above and including the layer in which the maximal image of a negative index is in $w$ ($j+1$ if there is no image). An equivalent way to think of the layer number is that it is the number of gaps above the maximal image of the negative indices. This is also the same as $n+1-m$ with the notation from Definition \ref{def:tree}. When $w$ is clear from the context, we will write $z$ for the layer number. 
\end{itemize}

The following observations are easy but useful consequences of Lemma \ref{lem:ignore} together with elementary considerations about active sites.

\begin{lemma}\label{lem:activesites}
Let $\pi=1234$ or $\pi=2143$ and $w$ be the label of a vertex in $BT^j(\pi)$.
\begin{enumerate}
    \item Suppose a site is inactive w.r.t. inserting the maximal element among the images of negative indices to a layer. Then this insertion creates a pattern $\pi$ that involves the element we just inserted and no positive index with a negative image (nothing from the bottom right quadrant).
    \item  Fix a layer in which we are considering active sites for $w$. If we insert the new maximal image $\ell$ of the negative indices to some active site, then the new active sites after this insertion are a subset of the old ones (where we think of the site where we inserted $\ell$ to have split into two). Furthermore, if a previously active site becomes inactive, then inserting $\ell+1$ there would create a pattern involving $\ell$ and $\ell+1$, and no positive index with a negative image (nothing from the bottom right quadrant).
\end{enumerate}

\end{lemma}

\begin{proof}
Omitted.
\end{proof}


The plan for the rest of the derivation of the generating trees is to first describe succession rules while staying in the same layer, then understand what happens when one passes from layer to layer, and finally combine the two into one succession rule. The next $3$ lemmas describe how some statistics of a permutation avoiding $\pi$ determine the same statistics for some of the successors.

\begin{lemma}\label{lem:2143layer}
Let the pattern we are avoiding be $\pi=2143$. Let $w$ be a signed permutation for which there are no images of negative indices above the $\ell$'th layer. Let $x$ be the number of elements before the first descent and $y$ be the number of active sites for insertion as the largest element of the $\ell$'th layer. If we just consider the successors of $w$ for which we perform an insertion in the $\ell$'th layer, then the pairs $(x,y)$ for each successor form the following multiset (in terms of the values of $x$ and $y$ for $w$):

\[\{ (2, y+1), (3, y+1), \ldots, (x+1, y+1), (x,x+1), (x, x+2), \ldots, (x,y)\}\]
\end{lemma}

\begin{proof}
All sites before the first descent in $w$ are active, as by Lemma \ref{lem:activesites}, the largest element we add would have to be involved in $2143$, and it cannot be $4$ or $3$ as it comes before the previous first descent, so there would be no $21$, and it also cannot be a $2$ or a $1$ as the elements larger than it form an increasing sequence by Lemma \ref{lem:struc}, so there would be no $43$.

If we insert to a site before the first descent, then there is a descent right after the inserted element, so the new number of sites before the first descent is $1$ more than the number of sites to the left of the insertion. All previously active sites stay active, since sites to the left of the last insertion are still before the first descent, and as for sites to the right of the last insertion, for a site to become inactive inserting there  would have to create a $2143$ involving both elements that were last added (by Lemma \ref{lem:activesites}). As the two elements last added are adjacent images with the smaller coming first, the only option is for them to be $2$ and $3$ in $2143$, but then there is no $4$ between them. So all active sites remain active in that case. This case gives the successor labels $(2,y+1), (3,y+1), \ldots, (x+1, y+1)$.

If we insert to a site after the first descent, then the number of sites before the first descent is unchanged. All sites after the first descent but to the left of the insertion become inactive, as inserting there would create an obvious $2143$. All sites to the right of the insertion stay active, as by Lemma \ref{lem:activesites} for one to become inactive, inserting there would have to create a $2143$ involving both last added elements, but as these are adjacent images, they would have to be the $2$ and $3$ in $2143$. There is no $4$ between them, so such a $2143$ cannot be formed. This case gives the successor labels $(x, x+1), (x, x+2), \ldots, (x,y)$.

Observe that the two cases together give the desired successor set.

\end{proof}


\begin{lemma}\label{lem:1234toplayer}
Let the pattern we are avoiding be $\pi=1234$. Let us consider inserting the new largest element to the top layer. Let $x$ be the number of elements before the first ascent and $y$ be the number of active sites for top layer. If we just consider the successors of $w$ for which we perform an insertion in the top layer, then the pairs $(x,y)$ for each successor form the following multiset (in terms of the values of $x$ and $y$ for $w$):

\[\{ (2, y+1), (3, y+1), \ldots, (x+1, y+1), (x,x+1), (x, x+2), \ldots, (x,y)\}\]
\end{lemma}

\begin{proof}
All sites before the first ascent in $w$ are active, as by Lemma \ref{lem:activesites}, the largest element we add would have to be involved in $1234$, and it is the largest element in the permutation (as we are inserting into the top layer), so it would have to be a $4$. But if there is no ascent before it, then no $12$ can be found before it, so it cannot be involved in a $1234$. 

If we insert the largest element into the first position, then the new first ascent is at $x+1$. It is obvious from Lemma \ref{lem:activesites} that all sites stay active. So this case gives the successor label $(x+1, y+1)$.

If we insert the largest element into some other position before the first ascent, then the new positions before the first ascent are exactly the sites preceding our inserted element. By what we argued before, all these also stay active. All active sites after the insertion also stay active, as Lemma \ref{lem:activesites} implies that for one to become active, there would need to be a $12$ before the insertion, but this is not the case. Hence, this case gives the successors $(2,y+1), (3,y+1),\ldots, (x,y+1)$.

If we insert the largest element into some active site after the first ascent, the position of the first ascent is unchanged. It is clear that all sites after it become inactive because inserting there would create a $1234$ from the ascent and the last two insertions. It is also clear from Lemma \ref{lem:activesites} that all active sites to the left of the insertion remain active. Hence, this case gives the successors $(x,x+1), (x,x+2), \ldots, (x,y)$.

Taking the union of the successor multisets from the three cases indeed gives the desired multiset.
\end{proof}

\begin{lemma}\label{lem:1234layer}
Let the pattern we are avoiding be $\pi=1234$. Let us consider inserting the new largest element to a layer which is not the top layer. Let $x$ be the number of sites before the first ascent. If we just consider the successors of $w$ for which we perform an insertion in this layer, then the positions of the first ascent form the following multiset (in terms of the value of $x$ for $w$):

\[\{ 2, 3, \ldots, x+1\}\]
\end{lemma}

\begin{proof}
All sites before the first ascent are active, since creating a new $1234$ would have at least 2 elements to one side of the inserted element, but having these on the left is impossible since it was inserted before the first ascent, and having these on the right is impossible by Lemma \ref{lem:struc}. All sites after the first ascent are inactive, because inserting there would create a $1234$ involving the first ascent as $12$, the inserted element as $3$, and the largest positive image of a positive index as $4$ (this is larger than the inserted element since we are inserting to a layer below the top layer).

After inserting to the first position, the new number of sites before the first ascent is $x+1$. After inserting into some other site before the first ascent, the sites before the first ascent are the sites to the left of the insertion, giving the terms $2,3,\ldots, x$. We see that the labels of successors are what is given in the lemma.
\end{proof}

The following lemmas give a characterization of the number of active sites as one switches from one layer to a layer above it.

\begin{lemma}\label{lem:2143switch}
Let the pattern we are avoiding be $\pi=2143$. $w$ is a signed permutation avoiding $\pi$, for which the number of sites before the first descent is $x$. Consider a layer such that there are currently only elements inserted to layers below it. Then the number of active sites w.r.t. inserting to this layer is $x$.
\end{lemma}

\begin{proof}
It is enough to show that the active sites are precisely those before the first descent. Any site after the first descent is inactive, as adding a site after a descent means we create a pattern involving the $2$ elements in the first descent as $21$, the new added element as $4$, and the positive index positive image at which the new layer starts as $3$. The sites before the first descent are all active, since the new largest element we add could only appear as $4$ or $3$ in a pattern $2143$ (because by Lemma \ref{lem:struc} everything larger than our maximal element forms an increasing sequence), and if we add a new largest element to one of the sites that are not after the first descent, there is no $21$ before it to complete the $2143$. Hence, the number of active sites is $x$.
\end{proof}

\begin{lemma}\label{lem:1234switchtotop}
Let the pattern we are avoiding be $\pi=1234$. $w$ is a signed permutation avoiding $\pi$. If there are currently no elements in the top layer, then for inserting to the top layer, all sites are active.
\end{lemma}

\begin{proof}
Suppose there is an inactive site in the top layer. For this to be inactive but $w$ to avoid $\pi$, inserting to that site must create a $1234$. By Lemma \ref{lem:ignore}, we also created a $1234$ even if we ignore the bottom right quadrant. The only change in the other 3 quadrants is the insertion of the new maximal element in the top layer, so there must be a $1234$ involving that element. This is the largest image among all the images (as it is in the top layer), so it must be a $4$ in the $1234$. Hence, there is a $123$ before it, but even without inserting the new largest element, the largest positive image of a positive index is greater than all previous images and comes after the $123$, so it also fulfils the role of the $4$, completing this $1234$. Hence, $w$ contains a $1234$, which is a contradiction. So all sites in the top layer are active.
\end{proof}

We now have all the ingredients to write down the succession rule for $BT^j(2143)$. The statistics we will keep track of for $2143$ are the following:
\begin{itemize}
    \item $x$ -- the number of sites before the first descent
    \item $y$ -- the number of active sites in the layer given by the current layer number, or in other words the number of active sites in the lowest layer to which the maximal image of the negative indices can be inserted
    \item $z$ -- the layer number.
\end{itemize}

\begin{proposition}\label{prop:suc2143}
The generating tree given by the following:
\begin{itemize}
    \item the label of the root is $(j+1, j+1, j+1)$.
    \item the succession function $suc$ that takes a label as its input and outputs the set of successors is defined recursively as follows:
    $$suc(x,y,z)=
    \begin{cases}
    0 &z=0,\\
    \{(2,y+1,z),(3,y+1,z),\ldots,(x+1,y+1,z)\\
    (x,x+1,z),(x,x+2,z),\ldots,(x,y,z)\}\bigcup suc(x,x,z{-}1) &z\geq1.
    \end{cases}$$
\end{itemize}

is isomorphic as a rooted tree to $BT^j(2143)$.
\end{proposition}

\begin{proof}
The only things we have to check is that if a signed permutation $w$ has the statistics $(x,y,z)$, then its successors have the statistics given in the lemma, and that the statistics of the root of $BT^j(2143)$ are the same as the label of the root given in the lemma. The latter is trivial, and as for the former, all the work is already done in Lemmas \ref{lem:2143layer} and $\ref{lem:2143switch}$. Lemma \ref{lem:2143layer} gives that the successors for fixed $z$ are those given in this lemma, and \ref{lem:2143switch} tells us what the labels are if we consider the layer below. Inducting on $z$ gives that this succession rule works.
\end{proof}

\begin{example}Figure \ref{fig:2143} shows the point graph of the $2143$ avoiding signed permutation
\[\begin{matrix}-6 & -5 & -4 & -3 & -2 & -1 & 1 & 2 & 3 & 4 & 5 & 6 \\ -6 & 4 & -3 & 5 & 2 & 1 & -1 & -2 & -5 & 3 & -4 & 6 \end{matrix} .\]
In each layer (horizontal strip), the active sites are shown with a cross. The relevant statistics $x,y,z$ are also displayed.
\begin{figure}[h!]
\centering
\begin{tikzpicture}[scale=0.6]
\draw[very thick](0,-7)--(0,8);
\draw[very thick](-8,0)--(8,0);
\node at (-1,1) {$\bullet$};
\node at (-2,2) {$\bullet$};
\node at (-5,4) {$\bullet$};
\node at (-3,5) {$\bullet$};
\node at (-4,-3) {$\bullet$};
\node at (-6,-6) {$\bullet$};
\node at (4,3) {$\bullet$};
\node at (6,6) {$\bullet$};
\draw(-7,6)--(6,6);
\draw(-7,3)--(4,3);
\draw[dashed](-6,-7)--(-6,7);
\draw[dashed](-5,-7)--(-5,7);
\draw[dashed](-4,-7)--(-4,7);
\draw[dashed](-3,-7)--(-3,7);
\draw[dashed](-2,-7)--(-2,7);
\draw[dashed](-1,-7)--(-1,7);
\node at (-6.5,5.5) {$\times$};
\node at (-5.5,5.5) {$\times$};
\node at (-4.5,5.5) {$\times$};
\node at (-2.5,5.5) {$\times$};
\node at (-1.5,5.5) {$\times$};
\node at (-6.5,6.5) {$\times$};
\node at (-5.5,6.5) {$\times$};
\node at (-4.5,6.5) {$\times$};
\node at (-8.2,4.5) {$z=$};
\node (z3) at (-7.5,1.5) {3};
\node (z2) at (-7.5,4.5) {2};
\node (z1) at (-7.5,6.5) {1};
\draw[->] (z3)--(z2);
\draw[->] (z2)--(z1);
\node at (1,5.5) {$y=5$};
\node at (5,4.5) {$j=2$};
\draw [decorate,decoration={brace,amplitude=5pt}]
(-7,7) -- (-4,7) node [black,midway,yshift=10pt] {$x=3$};
\end{tikzpicture}
\caption{The point graph of a 2143 avoiding signed permutation with active sites and statistics}
\label{fig:2143}
\end{figure}
\end{example}

We also have the ingredients to write down the succession rule for $BT^j(1234)$. The statistics we will keep track of for $1234$ are the following:
\begin{itemize}
    \item $x$ -- the number of sites before the first ascent
    \item $y$ -- the number of active sites in the top layer (by Lemma \ref{lem:1234switchtotop}, all sites are active before getting to the top layer, so this just increases by one each step as long as nothing has been inserted in the top layer yet)
    \item $z$ -- the layer number.
\end{itemize}
\begin{proposition}\label{prop:suc1234}
The generating tree given by the following:
\begin{itemize}
    \item the label of the root is $(j+1, j+1, j+1).$
    \item the succession function $suc$ that takes a label as its input and outputs the set of successors is defined recursively as follows:
    $$suc(x,y,z)=
    \begin{cases}
    \{(2,y+1,z),(3,y+1,z),\ldots,(x+1,y+1,z)\\
    (x,x+1,z),(x,x+2,z),\ldots,(x,y,z)\} &z=1,\\
    \{(2,y+1,z),(3,y+1,z),\ldots,(x+1,y+1,z)\}\\
    \bigcup suc(x,y,z-1) &z\geq2.
    \end{cases}$$
\end{itemize}
is isomorphic as a rooted tree to $BT^j(1234)$.
\end{proposition}

\begin{proof}
The proof is analogous to the proof of Proposition \ref{prop:suc2143}.
\end{proof}

\begin{example} Figure \ref{fig:1234} shows the point graph of $1234$ avoiding signed permutation
\[\begin{matrix}-6 & -5 & -4 & -3 & -2 & -1 & 1 & 2 & 3 & 4 & 5 & 6 \\ 2 & -3 & 4 & -5 & 1 & -6 & 6 & -1 & 5 & -4 & 3 & -2 \end{matrix} .\]
In each layer, the active sites are shown with a cross. The relevant statistics $x,y,z$ are also displayed.
\begin{figure}[h!]
\centering
\begin{tikzpicture}[scale=0.6]
\node at (-2,1) {$\bullet$};
\node at (-6,2) {$\bullet$};
\node at (-4,4) {$\bullet$};
\node at (-1,-6) {$\bullet$};
\node at (-3,-5) {$\bullet$};
\node at (-5,-3) {$\bullet$};
\node at (1,6) {$\bullet$};
\node at (3,5) {$\bullet$};
\node at (5,3) {$\bullet$};
\draw[very thick](0,-7)--(0,8);
\draw[very thick](-8,0)--(8,0);
\draw(-7,6)--(1,6);
\draw(-7,5)--(3,5);
\draw(-7,3)--(5,3);
\draw[dashed](-6,-5)--(-6,7);
\draw[dashed](-5,-5)--(-5,7);
\draw[dashed](-4,-5)--(-4,7);
\draw[dashed](-3,-7)--(-3,7);
\draw[dashed](-2,-7)--(-2,7);
\draw[dashed](-1,-7)--(-1,7);
\node at (-6.5,4.5) {$\times$};
\node at (-5.5,4.5) {$\times$};
\node at (-4.5,4.5) {$\times$};
\node at (-6.5,5.5) {$\times$};
\node at (-5.5,5.5) {$\times$};
\node at (-4.5,5.5) {$\times$};
\node at (-6.5,6.5) {$\times$};
\node at (-5.5,6.5) {$\times$};
\node at (-4.5,6.5) {$\times$};
\node at (-3.5,6.5) {$\times$};
\node at (-2.5,6.5) {$\times$};
\node at (-1.5,6.5) {$\times$};
\node at (-0.5,6.5) {$\times$};
\node at (5,5) {$j=3$};
\node at (-3.5,7.5) {$y=7$};
\draw [decorate,decoration={brace,amplitude=5pt}]
(-4,-5.5) -- (-7,-5.5) node [black,midway,yshift=-10pt] {$x=3$};
\node at (-8.2,4) {$z=$};
\node (z3) at (-7.5,4) {3};
\node (z2) at (-7.5,5.5) {2};
\node (z1) at (-7.5,6.5) {1};
\node (z4) at (-7.5,1.5) {4};
\draw[->] (z4)--(z3);
\draw[->] (z3)--(z2);
\draw[->] (z2)--(z1);
\end{tikzpicture}
\caption{The point graph of a $1234$ avoiding permutation with active sites and statistics}
\label{fig:1234}
\end{figure}

\end{example}

These generating trees turn the problem of counting permutations avoiding certain patterns into the problem of counting lattice paths of some length in $\mathbb{Z}^3$ given by the succession rules.
